Smoothing splines with some discontinuities

We generalize cubic smoothing splines to signals with a finite number of discontinuities at unknown positions. Rather than changing the roughness penalty, we deform the domain over which it is computed: every interval between consecutive observations can be stretched by a non-negative warp, subject to a total budget, and the optimizer spends the budget only where a jump makes stretching cheaper than bending. The estimator inherits the state-space form of smoothing splines, so it can be fitted by maximum likelihood with the Kalman filter, and it also admits a fast alternating algorithm that solves a banded linear system and takes a projected-gradient step on the warps. The budget is selected by an extended Bayesian information criterion whose constant is calibrated by simulation. In a Monte Carlo comparison the new estimators reconstruct a piecewise-smooth signal more accurately than the cubic smoothing spline with discontinuities of Storath and Weinmann, at the cost of more false alarms. Two energy applications illustrate the method: the temperature response of electricity demand in Northern Italy, and retail fuel prices, whose discontinuities, changes in excise duties, are dated by public record. The three supplements follow the references.

==> main-labels.tex <==
\newlabel{P-sec:intro}{{1}{2}{}{}{}}
\newlabel{P-sec:methodology}{{2}{4}{}{}{}}
\newlabel{P-sec:idea}{{2.1}{4}{}{}{}}
\newlabel{P-eq:objective}{{1}{4}{}{}{}}
\newlabel{P-sec:statespace}{{2.2}{5}{}{}{}}
\newlabel{P-fig:example_timewarp}{{1}{6}{}{}{}}
\newlabel{P-eq:stateSpace}{{2}{6}{}{}{}}
\newlabel{P-sec:atw}{{2.3}{7}{}{}{}}
\newlabel{P-eq:ki}{{3}{7}{}{}{}}
\newlabel{P-eq:grad}{{4}{9}{}{}{}}
\newlabel{P-sec:tuning}{{2.4}{9}{}{}{}}
\newlabel{P-eq:ebic}{{5}{10}{}{}{}}
\newlabel{P-tab:xi_fixed}{{1}{11}{}{}{}}
\newlabel{P-sec:simulations}{{3}{12}{}{}{}}
\newlabel{P-tab:rmse}{{2}{13}{}{}{}}
\newlabel{P-fig:sim_combined}{{2}{14}{}{}{}}
\newlabel{P-fig:sim_biasmse}{{3}{15}{}{}{}}
\newlabel{P-sec:applications}{{4}{16}{}{}{}}
\newlabel{P-sec:elettro}{{4.1}{16}{}{}{}}
\newlabel{P-tab:detection}{{3}{17}{}{}{}}
\newlabel{P-fig:elettro}{{4}{18}{}{}{}}
\newlabel{P-sec:carburanti}{{4.2}{19}{}{}{}}
\newlabel{P-tab:excise_dates}{{4}{20}{}{}{}}
\newlabel{P-fig:carburanti}{{5}{22}{}{}{}}
\newlabel{P-sec:conclusion}{{5}{24}{}{}{}}

